Learning Multi-modal Similarity

In many applications involving multi-media data, the definition of similarity between items is integral to several key tasks, e.g., nearest-neighbor retrieval, classification, and recommendation. Data in such regimes typically exhibits multiple modalities, such as acoustic and visual content of video. Integrating such heterogeneous data to form a holistic similarity space is therefore a key challenge to be overcome in many real-world applications. We present a novel multiple kernel learning technique for integrating heterogeneous data into a single, unified similarity space. Our algorithm learns an optimal ensemble of kernel transfor- mations which conform to measurements of human perceptual similarity, as expressed by relative comparisons. To cope with the ubiquitous problems of subjectivity and inconsistency in multi- media similarity, we develop graph-based techniques to filter similarity measurements, resulting in a simplified and robust training procedure.

==> 3-embedding.tex <==
% 1. 
%   Give some better justification of the mvu objective here:
%       More clearly explain the “assume dissimilar” idea
%       Illustrate with an example: if we have a total order of points on the line, we can recreate that. As edges are randomly deleted, we have less information, and more dimensions. In the limit, there is no information, and everything is equally far from everything else (n-sphere). Trace minimization, on the other hand, would prefer to collapse points together. This can probably be put across in one figure, but I think it's worth doing.

As a first step toward our goal of constructing an embedding algorithm for heterogeneous data, we first consider the case where the data has no feature
representation at all, and is entirely characterized by similarity measurements.  This situation often arises in psychometric experiments,
\eg,~\cite{gnmds}.

Without an explicit representation of $\X$, our goal is find a map $g:\X\rightarrow\R^n$ that respects a partial order
$\C$ over pairwise similarity measurements.  Assuming $\C$ is a partial order, it is possible to find an embedding that satisfies all constraints (see
Appendix~\ref{sec:diameter}).  In practice, $\C$ is often incomplete, so not all possible comparisons are observed.  Thus, to produce a 
unique solution, we must specify an objective function to optimize within the set of admissible embeddings.

If we consider the inner-product matrix of the embedded data $A$, \ie,
\[
A_{ij} = \langle g(x_i), g(x_j) \rangle,
\]
then one natural choice for the objective is to minimize the rank of $A$, or equivalently, the dimensionality of the embedding $g$.  Unfortunately, 
direct minimization of dimensionality is difficult in practice, and in fact, NP-Hard for this particular problem (see Section~\ref{sec:nphard}).  It is 
common to instead minimize $\trace(A)$, which is the convex envelope of the rank~\citep{boyd04}.
However, in the case of missing similarity measurements, there may not be enough structure in $\C$ to prevent $g$ from crowding or collapsing 
distinct points onto each-other.

Alternatively, we can design the embedding to maintain identifiability of points by maximizing distances:
\[
\max \sum_{i,j} \|g(x_i) - g(x_j)\|^2.
\]
This objective has also been used for manifold learning problems, where it is known as Maximum Variance Unfolding (MVU)~\citep{weinberger04}.
To ensure that the objective is bounded, it suffices to bound the diameter of the embedding.  Unlike manifold learning problems, we 
do not assume the existence of a neighborhood graph, so we cannot deduce an implicit diameter bound.  However, in Appendix~\ref{sec:diameter},
we derive an explicit bound on the diameter, thereby resolving scale-invariance of the solution.

To resolve translation invariance of the embedding, we restrict $A$ to be centered, \ie,
\[
\one\trans A\one = 0.
\]
Note that the matrix of (squared) Euclidean distances between embedded points can be expressed algebraically as
\[
\Delta = \diag(A)\one\trans + \one\diag(A)\trans - 2A.
\]
As in MVU, these two equations lead to a simpler form of the objective:
\begin{align*}
\sum_{i,j} \|g(x_i) - g(x_j)\|^2 = \one\trans \Delta \one &= \one\trans \left( \diag(A)\one\trans + \one\diag(A)\trans - 2A \right) \one\\
&= \trace(A)\one\trans\one + \one\trans\one\trace(A) - 2 (\one\trans A \one)\\
&= 2n\trace(A) \propto \trace(A).
\end{align*}
In other words, maximizing $\trace(A)$ is equivalent to maximizing the sum of all pairwise distances.

The diameter bound from Lemma~\ref{lem:diameter} (Appendix~\ref{sec:diameter}) indicates that a solution exists inside an $n$-dimensional ball of fixed diameter.  Since the embedding is
also constrained to be centered at the origin, we can equivalently bound the radius of the data, which in this case, corresponds to the norms $A_{ii}$.

By combining the MVU objective with the diameter bound, margin constraints, and the centering constraint, we arrive at
Algorithm~\ref{alg:poe}.  Note that the objective function is linear in $A$, and the constraints can be expressed as linear matrix inequalities.  

\begin{algorithm}
\caption{Partial order embedding (POE)}\label{alg:poe}%
\begin{algorithmic}
    \STATE {\bfseries Input:} $n$ objects $\X=\{x_1,x_2,\dots,x_n\}$, partial order $\C$
    \STATE {\bfseries Output:} mapping $g:\X\rightarrow \R^n$
    \begin{align*}
        \max_{A} ~~~ \trace(A)\\
%         A_{ii} + A_{jj} - 2A_{ij} & \leq (2n +1)\diam(\C) &   \forall i,j \in \X \\
        A_{ii} + A_{jj} - 2A_{ij} + 1 & \leq A_{kk} + A_{\ell\ell} - 2A_{k\ell}
        &\forall (i,j,k,\ell) \in \C\\
        \one\trans A\one &= 0\\
        2A_{ii} & \leq (2n +1)(\diam(\C)+1) &   \forall i \in \X \\
        A &\succeq 0
    \end{align*}
    \STATE Find the spectral decomposition: $A = V{\Lambda}V\trans$.
    \STATE For each $i\in\X$, define the embedding as $g(x_i) \doteq \left(\Lambda^{1/2}V\trans\right)_i$.
\end{algorithmic}
\end{algorithm}


% \subsection{Structure-preserving reductions}

% 4.
%   As a general result, we can embed any graph such that edge pairs have smaller distance than non-edge-pairs. Manifold learning definitely falls into this category of problem. In particular, all constraint graphs of this form are bipartite, so we are justified in rephrasing the problem using “choke” variables. I used this in the icml paper experiments, but never wrote it down.




